RoboMorph: In-Context Meta-Learning for Robot Dynamics Modeling

The landscape of Deep Learning has experienced a major shift with the pervasive adoption of Transformer-based architectures, particularly in Natural Language Processing (NLP). Novel avenues for physical applications, such as solving Partial Differential Equations and Image Vision, have been explored. However, in challenging domains like robotics, where high non-linearity poses significant challenges, Transformer-based applications are scarce. While Transformers have been used to provide robots with knowledge about high-level tasks, few efforts have been made to perform system identification. This paper proposes a novel methodology to learn a meta-dynamical model of a high-dimensional physical system, such as the Franka robotic arm, using a Transformer-based architecture without prior knowledge of the system's physical parameters. The objective is to predict quantities of interest (end-effector pose and joint positions) given the torque signals for each joint. This prediction can be useful as a component for Deep Model Predictive Control frameworks in robotics. The meta-model establishes the correlation between torques and positions and predicts the output for the complete trajectory. This work provides empirical evidence of the efficacy of the in-context learning paradigm, suggesting future improvements in learning the dynamics of robotic systems without explicit knowledge of physical parameters. Code, videos, and supplementary materials can be found at project website. See https://sites.google.com/view/robomorph/

==> Scripts/Algorithms/dexpbt.tex <==
\begin{algorithm}[t]
\caption{\textsc{MUTATE} subroutine in DexPBT \cite{petrenko2023dexpbt}}\label{algo:dexpbt}

\SetAlgoLined
\DontPrintSemicolon

\KwIn{Parent hyperparameters $h^*$}
\KwOut{Mutated hyperparameters $h$}

\SetKwFunction{FMain}{\textsc{MUTATE}}
\SetKwProg{Fn}{Function}{}{}

\Fn{\FMain{$h^*$}}{
    \ForEach{$i \in 1 \ldots n$}{
        $z \gets \mathcal U(0, 1)$\;
        \If{$z < \beta_{mut}$}{
            $\mu \gets \mathcal U(\mu_{min}, \mu_{max})$\;
            $d \gets \mathcal U(0, 1)$\;
            \eIf{$d < 0.5$}{
                $h_i \gets h_i * \mu$\;
            }{
                $h_i \gets h_i / \mu$\;
            }
        }
    }
}\textbf{end}

\end{algorithm}

==> Scripts/Algorithms/mutate.tex <==
\begin{algorithm}[t]
\caption{\textsc{Mutate} subroutine in PBRL}\label{algo:mutate}

\SetAlgoLined
\DontPrintSemicolon

\KwIn{Parent hyperparameters $h^*$}
\KwOut{Mutated hyperparameters $h$}

\SetKwFunction{FMain}{\textsc{Mutate}}
\SetKwProg{Fn}{Function}{}{}

\Fn{\FMain{$h^*$}}{
    \For{$i \gets 1, \ldots, n$}{
        $\delta \gets \mathcal U(\delta_{min}, \delta_{max})$\;
        $h_i \gets \text{clip}(\delta h_i^*, h_{i,min}, h_{i,max})$\;
    }
}\textbf{end}

\end{algorithm}

==> Scripts/Algorithms/pbrl.tex <==
\begin{algorithm}[t]
\caption{PBRL algorithm}\label{algo:pbrl}

\SetAlgoLined
\DontPrintSemicolon

\KwIn{Initial population $\mathcal{P}$ of agents ($\Theta$ random, $\bm h$ sampled from a uniform distribution)}
\KwOut{Updated population}

$N_{iter} = 0$\;
\While{not end of training}{
    $\theta \gets \textsc{Train} (\Pi(\Theta, \bm h))$\;
    $N_{iter} = N_{iter} + 1$\;
    \If{$N_{iter} > N_{start}$ and $ N_{iter}$ \% $N_{evo} = 0$}{
        \ForEach{\text{agent} $\pi(\theta, h) \in \mathcal P$}{
            $\mathcal{R}_{mean} \gets \textsc{Eval} (\pi(\theta, h))$\;
            Sort $\pi(\theta, h)$ based on $\mathcal{R}_{mean}$\;
        }
        Partition $\mathcal P$ into $\mathcal P_{top\,25\,\%}$, $\mathcal P_{mid\,50\,\%}$, $\mathcal P_{bottom\,25\,\%}$ \;
        Sample $\pi^*(\theta^*, h^*)$ from $\mathcal{P}_{top\,25\,\%}$ at random\;
        \ForEach{\text{agent} $\pi(\theta, h) \in \mathcal{P}_{bottom\,25\,\%}$}{
            $\pi(\theta) \gets \pi^*(\theta^*)$\;
            $h \gets \textsc{Mutate} (h^*)$\;
        }
    }
}

\end{algorithm}

==> Scripts/Figures/approach.tex <==
\begin{comment}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/approach.png}
    \captionsetup{width=\textwidth}
    \caption{PBRL framework used to learn robotic manipulation tasks through a combination of RL, evolutionary selection, and GPU-based parallel simulations.}
    \label{fig:approach}
\end{figure*}
\end{comment}


% Size of blocks (learning and simulation)
\newlength{\blockwidth}
\setlength{\blockwidth}{0.4\textwidth}
\newlength{\blockheight}
\setlength{\blockheight}{0.8\blockwidth}

% Height of inner block
\newlength{\innerheight}
\setlength{\innerheight}{0.75\blockheight}

% Horizontal offset: how much the left side of inner block is offset wrt the left side of outer block
\newlength{\ho}
\setlength{\ho}{0.025\blockwidth}

% Vertical offset: how much the bottom side of inner block is offset wrt the bottom side of outer block
\newlength{\vo}
\setlength{\vo}{0.05\blockheight}

% Width of the arrows between inner blocks
\newlength{\arrowwidth}
\setlength{\arrowwidth}{0.15\blockwidth}

% Width of inner blocks
\newlength{\innerwidth}
\setlength{\innerwidth}{\dimexpr 0.5\blockwidth - \ho - 0.5\arrowwidth \relax}

% Center of blocks (in absolute coordinates wrt to block center)
\newlength{\innerblockcx}
\setlength{\innerblockcx}{\dimexpr 0.5\arrowwidth + 0.5\innerwidth \relax}
\newlength{\innerblockcy}
\setlength{\innerblockcy}{\dimexpr 0.5\blockheight - \vo - 0.5\innerheight} \relax

% Bottom-left corner of left block (agents)
\newlength{\innerblockblx}
\setlength{\innerblockblx}{\dimexpr -\innerblockcx -0.5\innerwidth \relax}
\newlength{\innerblockbly}
\setlength{\innerblockbly}{\dimexpr -\innerblockcy -0.5\innerheight \relax}

% Text offset
\newlength{\textoffset}
\setlength{\textoffset}{\dimexpr 0.5\blockheight - 0.5\vo - 0.5\innerheight \relax}

% Image size
\newlength{\imagewidth}
\settowidth{\imagewidth}{\includegraphics{Figures/anymal.png}}
\newlength{\imageheight}
\settoheight{\imageheight}{\includegraphics{Figures/anymal.png}}

% How much the image must be trimmed to fit in the inner block
\newlength{\widthtotrim}
\setlength{\widthtotrim}{\innerwidth * \ratio{\imageheight}{\innerheight}}
\newlength{\lefttrim}
\setlength{\lefttrim}{260pt}
\newlength{\righttrim}
\setlength{\righttrim}{\dimexpr \imagewidth - \lefttrim - \widthtotrim \relax}

% Height of square inside Agents inner block
\newlength{\squareheight}
\setlength{\squareheight}{0.6\innerheight}

% Width of square inside Agents inner block
\newlength{\squarewidth}
\setlength{\squarewidth}{\dimexpr \innerwidth - 2\ho \relax}

% Center of square
\newlength{\squarecx}
\setlength{\squarecx}{-\innerblockcx}
\newlength{\squarecy}
\setlength{\squarecy}{\dimexpr -\innerblockcy -0.5\innerheight +\ho + 0.5\squareheight \relax}

% Bottom-left corner of square block (agents)
\newlength{\squareblx}
\setlength{\squareblx}{\dimexpr \squarecx -0.5\squarewidth \relax}
\newlength{\squarebly}
\setlength{\squarebly}{\dimexpr \squarecy -0.5\squareheight \relax}

% Policies text offset
\newlength{\ptextoffset}
\setlength{\ptextoffset}{\dimexpr 0.5\innerheight - 0.5\squareheight - 0.5\ho \relax}

% Ranking block size
\newlength{\rankingblockwidth}
\setlength{\rankingblockwidth}{0.65\blockwidth}
\newlength{\rankingblockheight}
\setlength{\rankingblockheight}{\innerheight}

% Transfer block size
\newlength{\transferblockwidth}
\setlength{\transferblockwidth}{0.2\blockwidth}
\newlength{\transferblockheight}
\setlength{\transferblockheight}{0.7\rankingblockheight}

% Mutate block size
\newlength{\mutateblockwidth}
\setlength{\mutateblockwidth}{\transferblockwidth}
\newlength{\mutateblockheight}
\setlength{\mutateblockheight}{0.25\transferblockheight}

\tikzstyle{block} = [draw, very thick, rounded corners=10pt, rectangle, minimum width=\blockwidth, minimum height=\blockheight]

\begin{figure*}[t]
\centering
\begin{tikzpicture}[auto,>=latex']
    % Learning block
    \node [block] (learning) {};
    \node [above, font=\normalsize] at (learning.north) {LEARNING (Section~\ref{sec:rl})};
    \node [font=\normalsize] at ([xshift=-\innerblockcx, yshift=-\textoffset] learning.north) {Agents};
    \node [font=\normalsize] at ([xshift=+\innerblockcx, yshift=-\textoffset] learning.north) {Simulation};
    \draw [black, thick] (learning) ++(\innerblockblx, \innerblockbly) rectangle ++(\innerwidth, \innerheight) node (agents) {};
    \node[inner sep=0pt] (simulation) at ([xshift=\innerblockcx, yshift=-\innerblockcy] learning.center) {\includegraphics[width=\innerwidth, height=\innerheight, trim=\lefttrim{} 0 \righttrim{} 0, clip]{Figures/anymal.png}};  %trim options: lbrt

    % Learning arrows
    \draw [->, thick] ([yshift=-1/3*\innerheight] agents.center) -- ([yshift=0.5\innerheight-1/3*\innerheight] simulation.west) node [midway, font=\large] {$a_t$};
    \draw [->, thick] ([yshift=-0.5\innerheight+1/3*\innerheight] simulation.west) -- ([yshift=-2/3*\innerheight] agents.center) node [midway, font=\large, align=center] {$s_t, r_t$};

    % Policies square
    \draw [black] (learning) ++(\squareblx, \squarebly) rectangle ++(\squarewidth, \squareheight) node[xshift=-0.5\squarewidth, yshift=-0.5\squareheight, align=center, font=\normalsize] (policies) {$\pi_0(\theta_0, h_0)$\\$\vdots$\\$\pi_n(\theta_n,h_n)$};
    \node [align=center, font=\normalsize] at ([xshift=0, yshift=0.5\squareheight+\ptextoffset] policies) {PPO, SAC,\\DPPG};

    % Evolution block
    \node [block, right of=learning, node distance=10cm] (evolution) {};
    \node [above, font=\normalsize] at (evolution.north) {EVOLUTION (Section~\ref{sec:pbt})};
    \node [draw, rounded corners=10pt, rectangle, thick, minimum width=\rankingblockwidth, minimum height=\rankingblockheight] (ranking) at ([xshift=2\ho+0.5\rankingblockwidth, yshift=\innerblockbly+0.5\rankingblockheight] evolution.west) {};
    \node [draw, rounded corners=10pt, rectangle, thick, minimum width=\transferblockwidth, minimum height=\transferblockheight] (transfer) at ([xshift=-2\ho-0.5\transferblockwidth, yshift=\innerblockbly+\innerheight-0.5\transferblockheight] evolution.east) {};
    \node [draw, rounded rectangle, font=\normalsize, minimum height=\mutateblockheight] (mutate) at ([xshift=0.5\blockwidth-2\ho-0.5\transferblockwidth, yshift=-0.5\blockheight+\vo+0.5\mutateblockheight] evolution) {Mutate};
    \node [font=\normalsize] at ([xshift=-0.5\blockwidth+2\ho+0.5\rankingblockwidth, yshift=-\textoffset] evolution.north) {Ranking};
    \node [font=\normalsize] at ([xshift=0.5\blockwidth-2\ho-0.5\transferblockwidth, yshift=-\textoffset] evolution.north) {Transfer};

    % Ranking block
    \node [draw, rectangle, rounded corners=10pt, minimum width=0.8\rankingblockwidth, minimum height=0.25\rankingblockheight, font=\normalsize] (bottomagents) at ([yshift=0.3\rankingblockheight] ranking) {Agents bottom 25\%};
    \node [draw, rectangle, rounded corners=10pt, minimum width=0.8\rankingblockwidth, minimum height=0.25\rankingblockheight, font=\normalsize] (midagents) at (ranking) {Agents mid 50\%};
    \node [draw, rectangle, rounded corners=10pt, minimum width=0.8\rankingblockwidth, minimum height=0.25\rankingblockheight, font=\normalsize] (topagents) at ([yshift=-0.3\rankingblockheight] ranking) {Agents top 25\%};

    % Transfer block
    \node [draw, rectangle, minimum width=0.5\transferblockwidth, font=\large] (hyperparameters) at ([yshift=0.5\transferblockheight-0.5\rankingblockheight] transfer) {$h^*$};
    \node [font=\normalsize] (parameters) at ([yshift=-0.5\transferblockheight+0.5\rankingblockheight] transfer) {$\theta^*$};
            
    % Arrows
    \draw[->, very thick] ([yshift=0.5\blockheight-\vo-0.2\rankingblockheight] learning.east) -- node[font=\normalsize, anchor=north] {$\mathcal R_{mean}$} ([yshift=0.5\blockheight-\vo-0.2\rankingblockheight] evolution.west);
    \draw [->, very thick] (evolution) -- node[name=back] {} (learning);
    \draw [->, very thick] (topagents.west) -- node[align=center, pos=0.6, font=\normalsize, anchor=south] (return) {Continue Learning} ([yshift=-0.5\blockheight+\vo+0.2\rankingblockheight] learning.east);
    \node [right of=topagents, node distance=0.45\rankingblockwidth, coordinate, font=\scriptsize] (topagentseast) {};
    \draw [-, thick] (topagents.east) -- (topagentseast);
    \draw [->, thick] (topagentseast) |- ([yshift=-0.5\transferblockheight+0.2\rankingblockheight] transfer.west);
    \node [left of=topagents, node distance=0.45\rankingblockwidth, coordinate, font=\scriptsize] (topagentswest) {};
    \draw [-, very thick] (midagents.west) -| (topagentswest);
    \draw [->, thick] ([yshift=0.5\transferblockheight-0.2\rankingblockheight] transfer.west) -- (bottomagents.east);
    \draw [->, thick] (mutate.north) -- (hyperparameters.south);
\end{tikzpicture}
\caption{PBRL framework used to learn robotic manipulation tasks through a combination of RL, evolutionary selection, and GPU-based parallel simulations.}
\label{fig:approach}
\end{figure*}



==> Scripts/Figures/ddpg.tex <==
\begin{figure}[t]
    \centering

    % Legend
    \begin{center}
    \scriptsize{{\legblue}~DDPG \hspace{0.3em} \par {\legred}~PBRL-DDPG 4 agents \hspace{0.3em} {\leggreen}~PBRL-DDPG 8 agents}
    \end{center}

    % Figure
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/anymal-ddpg.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/shadow-ddpg.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/humanoid-ddpg.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-ddpg.png}
    \end{subfigure}
    
    % Caption
    \caption{Training results of baseline DDPG and PBRL-DDPG for $\lvert \mathcal P \rvert \in \{ 4, 8 \}$. The shaded area displays the performance between the best and the worst agent in $\mathcal P$, or among 4 different seeds in a non-evolutionary baseline.}
    \label{fig:ddpg}
\end{figure}

==> Scripts/Figures/envs.tex <==
\begin{figure}[t!]
\centering
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/anymal.JPG}
        \caption{\textit{Anymal Terrain}}
        \label{fig:anymal}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/shadow.png}
        \caption{\textit{Shadow Hand}}
        \label{fig:shadow-hand}
    \end{subfigure}
    \\ \vspace{0.125cm}
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/humanoid.png}
        \caption{\textit{Humanoid}}
        \label{fig:humanoid}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/franka_nut.png}
        \caption{\textit{Franka Nut Pick}}
        \label{fig:franka-nut-pick}
    \end{subfigure}
    \captionsetup{width=\columnwidth}
    \caption{Simulated experiments are performed on four Isaac Gym benchmark tasks: (\subref{fig:anymal}) \textit{Anymal Terrain}, to teach a quadruped robot to navigate uneven terrain; (\subref{fig:shadow-hand}) \textit{Shadow Hand}, which involves manipulating a cube to a desired orientation with a robot hand; (\subref{fig:humanoid}) \textit{Humanoid}, for bipedal locomotion; and (\subref{fig:franka-nut-pick}) \textit{Franka Nut Pick}, where the goal is to grasp and lift a hex nut from a random location on a work surface.}
    \label{fig:envs}
\end{figure}


==> Scripts/Figures/experiment.tex <==
\begin{figure}[t]
    \centering

    % Figure
    \begin{subfigure}[b]{0.32\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-nut-pick-real-1-nobg.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-nut-pick-real-2-nobg.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-nut-pick-real-3-nobg.png}
    \end{subfigure}
    
    % Caption
    \caption{Snapshots of the \textit{Franka Nut Pick} experiment on the real robot: full video at \url{https://sites.google.com/view/pbrl/}.}
    \label{fig:experiment}
\end{figure}

==> Scripts/Figures/mutation_comp.tex <==
\begin{figure*}[t!]
    \centering
    \begin{center}
    \scriptsize{{\legred}~Perturbation \hspace{0.3em} {\leggrey}~Uniform-Sampling \hspace{0.3em} {\leggreen}~DexPBT \cite{petrenko2023dexpbt}}
    \end{center}

    % Figure
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/anymal-ppo-mut.png}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.24\textwidth}
        \centering
    \includegraphics[width=\textwidth]{Figures/shadow-ppo-mut.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/humanoid-ppo-mut.png}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.24\textwidth}
        \centering
    \includegraphics[width=\textwidth]{Figures/franka-ppo-mut.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/anymal-ddpg-mut.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/shadow-ddpg-mut.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/humanoid-ddpg-mut.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-ddpg-mut.png}
    \end{subfigure}

    % Caption
    \caption{Comparison of different mutation schemes for PBRL-PPO (top) and PBRL-DDPG (bottom) with $\lvert \mathcal P \rvert = 4$.}
    \label{fig:mutation_comp}
\end{figure*}

==> Scripts/Figures/ppo.tex <==
\begin{figure}[b!]
    \centering

    % Legend
    \begin{center}
    \scriptsize{{\legblue}~PPO \hspace{0.3em} {\legred}~PBRL-PPO~4~agents \par {\leggreen}~PBRL\nobreakdash-PPO~8~agents \hspace{0.3em} {\legpurple}~PBRL-PPO~16~agents}
    \end{center}

    % Figure
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/anymal-ppo.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/shadow-ppo.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/humanoid-ppo.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-ppo.png}
    \end{subfigure}
    
    % Caption
    \caption{Training results of baseline PPO and PBRL-PPO for $\lvert \mathcal P \rvert \in \{ 4, 8, 16 \}$. The shaded area represents the performance between the best and the worst agent in $\mathcal P$, or among 4 different seeds in a non-evolutionary baseline.}
    \label{fig:ppo}
\end{figure}

==> Scripts/Figures/sac.tex <==
\begin{figure}[b!]
    \centering

    % Legend
    \begin{center}
    \scriptsize{{\legblue}~SAC \hspace{0.3em} {\legred}~PBRL-SAC 4 agents \hspace{0.3em} {\leggreen}~PBRL-SAC 8 agents}
    \end{center}

    % Figure
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/anymal-sac.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/shadow-sac.png}
    \end{subfigure}
    \\
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/humanoid-sac.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-sac.png}
    \end{subfigure}

    % Caption
    \caption{Training results of baseline SAC and PBRL-SAC for $\lvert \mathcal P \rvert \in \{ 4, 8 \}$. The shaded area displays the performance between the best and the worst agent in $\mathcal P$, or among 4 different seeds in a non-evolutionary baseline.}
    \label{fig:sac}
\end{figure}

==> Scripts/Figures/successes.tex <==
\begin{figure}[t]
    \centering

    % Legend
    \begin{center}
    \scriptsize{{\legblue}~PPO \hspace{0.3em} {\legred}~PBRL-PPO~4~agents \par
    {\leggreen}~PBRL\nobreakdash-PPO~8~agents \hspace{0.3em} {\legpurple}~PBRL-PPO~16~agents}
    \end{center}

    % Figure
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-succ-ppo.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/franka-succ-pbrl-ppo.png}
    \end{subfigure}
    
    % Caption
    \caption{Success rate of \textit{Franka Nut Pick} with PPO baseline and PBRL-PPO in simulation for $\lvert \mathcal P \rvert \in \{4, 8, 16\}$. The shaded area represents the performance between the best and the worst agent in $\mathcal P$, or among 4 different seeds in a non-evolutionary baseline.}
    \label{fig:successes}
\end{figure}

==> Scripts/Tables/ft_6.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{c|ccccc}
\hline
    & $R^2$ & RMSE & NRMSE & Fit Index \\ \hline
$x$ & \cellcolor{lightgreen!80}0.998 & \cellcolor{lightgreen!80}0.0083 & \cellcolor{lightgreen!80}0.0391 & \cellcolor{lightgreen!80}96.09 \\
$y$ & \cellcolor{lightgreen!80}1 & \cellcolor{lightgreen!80}0.0081 & \cellcolor{lightgreen!80}0.0211 & \cellcolor{lightgreen!80}97.89 \\
$z$ & \cellcolor{yellow!50}0.867 & \cellcolor{yellow!50}0.0212 & \cellcolor{yellow!50}0.3643 & \cellcolor{yellow!50}63.57 \\
$X$ & \cellcolor{lightgreen!80}0.999 & \cellcolor{lightgreen!80}0.0044 & \cellcolor{lightgreen!80}0.0244 & \cellcolor{lightgreen!80}97.56 \\
$Y$ & \cellcolor{lightgreen!80}1 & \cellcolor{lightgreen!80}0.0073 & \cellcolor{lightgreen!80}0.0196 & \cellcolor{lightgreen!80}98.04 \\
$Z$ & \cellcolor{yellow!50}0.953 & \cellcolor{yellow!50}0.0209 & \cellcolor{yellow!50}0.2163 & \cellcolor{yellow!50}78.37 \\
$W$ & \cellcolor{lightgreen!50}0.965 & \cellcolor{lightgreen!50}0.0117 & \cellcolor{lightgreen!50}0.1861 & \cellcolor{lightgreen!50}81.39 \\
$q_0$ & \cellcolor{lightgreen!80}1 & \cellcolor{lightgreen!80}0.0112 & \cellcolor{lightgreen!80}0.0129 & \cellcolor{lightgreen!80}98.71 \\
$q_1$ & \cellcolor{lightgreen!50}0.983 & \cellcolor{lightgreen!50}0.0277 & \cellcolor{lightgreen!50}0.132 & \cellcolor{lightgreen!50}86.8 \\
$q_2$ & \cellcolor{lightgreen!80}0.997 & \cellcolor{lightgreen!80}0.0075 & \cellcolor{lightgreen!80}0.0545 & \cellcolor{lightgreen!80}94.55 \\
$q_3$ & \cellcolor{lightgreen!50}0.969 & \cellcolor{lightgreen!50}0.0368 & \cellcolor{lightgreen!50}0.1756 & \cellcolor{lightgreen!50}82.44 \\
$q_4$ & \cellcolor{lightgreen!80}1 & \cellcolor{lightgreen!80}0.003 & \cellcolor{lightgreen!80}0.0213 & \cellcolor{lightgreen!80}97.87 \\
$q_5$ & \cellcolor{lightgreen!80}0.999 & \cellcolor{lightgreen!80}0.0046 & \cellcolor{lightgreen!80}0.0323 & \cellcolor{lightgreen!80}96.77 \\
$q_6$ & \cellcolor{lightgreen!80}1 & \cellcolor{lightgreen!80}0.0028 & \cellcolor{lightgreen!80}0.0195 & \cellcolor{lightgreen!80}98.05 \\
\hline
\end{tabular}
\caption{Fine-tuning 6 (2.5 Hours).}
\end{table}

==> Scripts/Tables/ft_9.tex <==
\begin{table}[H]
    \centering
    \scriptsize
    \begin{tabular}{c|ccccc}
        \hline
        & $R^2$ & RMSE & NRMSE & Fit Index \\
        \hline
        $x$ & \cellcolor{lightgreen!80}0.998 & \cellcolor{lightgreen!80}0.0083 & \cellcolor{lightgreen!80}0.0391 & \cellcolor{lightgreen!80}96.09 \\
        $y$ & \cellcolor{lightgreen!80}0.999 & \cellcolor{lightgreen!80}0.0088 & \cellcolor{lightgreen!80}0.023  & \cellcolor{lightgreen!80}97.7  \\
        $z$ & \cellcolor{red!30}-0.466 & \cellcolor{red!30}0.0706 & \cellcolor{red!30}1.2108 & \cellcolor{red!30}-21.08 \\
        $X$ & \cellcolor{lightgreen!80}0.998 & \cellcolor{lightgreen!80}0.0078 & \cellcolor{lightgreen!80}0.0438 & \cellcolor{lightgreen!80}95.62 \\
        $Y$ & \cellcolor{lightgreen!80}1     & \cellcolor{lightgreen!80}0.0055 & \cellcolor{lightgreen!80}0.0148 & \cellcolor{lightgreen!80}98.52 \\
        $Z$ & \cellcolor{orange!50}0.644 & \cellcolor{orange!50}0.0576 & \cellcolor{orange!50}0.5966 & \cellcolor{orange!50}40.34 \\
        $W$ & \cellcolor{orange!50}0.677 & \cellcolor{orange!50}0.0357 & \cellcolor{orange!50}0.568  & \cellcolor{orange!50}43.2  \\
        $q_0$ & \cellcolor{lightgreen!80}1     & \cellcolor{lightgreen!80}0.0091 & \cellcolor{lightgreen!80}0.0105 & \cellcolor{lightgreen!80}98.95 \\
        $q_1$ & \cellcolor{yellow!50}0.936 & \cellcolor{yellow!50}0.053  & \cellcolor{yellow!50}0.2523 & \cellcolor{yellow!50}74.77 \\
        $q_2$ & \cellcolor{lightgreen!80}0.998 & \cellcolor{lightgreen!80}0.0066 & \cellcolor{lightgreen!80}0.0478 & \cellcolor{lightgreen!80}95.22 \\
        $q_3$ & \cellcolor{orange!50}0.802 & \cellcolor{orange!50}0.0931 & \cellcolor{orange!50}0.4446 & \cellcolor{orange!50}55.54 \\
        $q_4$ & \cellcolor{lightgreen!80}0.999 & \cellcolor{lightgreen!80}0.0051 & \cellcolor{lightgreen!80}0.0363 & \cellcolor{lightgreen!80}96.37 \\
        $q_5$ & \cellcolor{lightgreen!80}0.995 & \cellcolor{lightgreen!80}0.0104 & \cellcolor{lightgreen!80}0.0725 & \cellcolor{lightgreen!80}92.75 \\
        $q_6$ & \cellcolor{lightgreen!80}0.999 & \cellcolor{lightgreen!80}0.004  & \cellcolor{lightgreen!80}0.0273 & \cellcolor{lightgreen!80}97.27 \\
        \hline
    \end{tabular}
    \caption{Fine-tuning 9 (5 Hours).}
\end{table}
